Verbing Weirds Language (Models): Evaluation of English Zero-Derivation in Five LLMs

Lexical-syntactic flexibility, in the form of conversion (or zero-derivation) is a hallmark of English morphology. In conversion, a word with one part of speech is placed in a non-prototypical context, where it is coerced to behave as if it had a different part of speech. However, while this process affects a large part of the English lexicon, little work has been done to establish the degree to which language models capture this type of generalization. This paper reports the first study on the behavior of large language models with reference to conversion. We design a task for testing lexical-syntactic flexibility -- the degree to which models can generalize over words in a construction with a non-prototypical part of speech. This task is situated within a natural language inference paradigm. We test the abilities of five language models -- two proprietary models (GPT-3.5 and GPT-4), three open-source models (Mistral 7B, Falcon 40B, and Llama 2 70B). We find that GPT-4 performs best on the task, followed by GPT-3.5, but that the open source language models are also able to perform it and that the 7B parameter Mistral displays as little difference between its baseline performance on the natural language inference task and the non-prototypical syntactic category task, as the massive GPT-4.

==> tables/difference_from_proto.tex <==
\begin{tblr}{lrrrrr}
  \toprule
  category & falcon & gpt-3.5 & gpt-4 & llama2 & mistral \\
  \midrule
  nonce words $-$ prototypical POS & -0.07 & -0.07 & -0.01 & -0.03 & -0.01 \\
  non-prototypical POS $-$ prototypical POS & -0.09 & -0.08 & -0.01 & -0.03 & -0.03 \\
  \bottomrule
\end{tblr}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../lrec-coling2024"
%%% End:


==> tables/frames_boring.tex <==
\begin{tabular}{lll}
  \toprule
  Subtask & Prompt & Intended\\
  \midrule
\multirow{6}{*}{transitive} & If I asked you to \{\} it, do I want you to \{\} it? & True\\
 & If I asked you to \{\} it, do I want you to not \{\} it? & False\\
 & If I asked you not to \{\} it, do I want you to \{\} it? & False\\
& If I asked you to not \{\} it, do I want you to not \{\} it? & True\\
 & If I say, “Don’t \{\} me,” am I asking you to not \{\} me? & True\\
 & If I say, “Don’t \{\} me,” am I asking you to \{\} me? & False\\
\midrule
\multirow{4}{*}{intransitive} & If I \{\} daily, do I \{\} every day? & True\\
 & If I don't \{\} daily, do I \{\} every day? & False\\
 & If I tried to \{\}, did I attempt to \{\}? & True\\
 & If I did not try to \{\}, did I attempt to \{\}? & False\\
\midrule
\multirow{4}{*}{count} & If I like this \{\} more than the other one, do I prefer this \{\} to the other one? & True\\
 & If I like this \{\} more than the other one. Do I prefer the other \{\} to this one? & False\\
 & If I like this \{\} less than the other one, do I prefer this \{\} to the other one? & False\\
 & If I like this \{\} less than the other one. Do I prefer the other \{\} to this one? & True\\
\midrule
\multirow{4}{*}{mass}& I prefer less \{\}. Do I prefer less \{\}? & True\\
 & I prefer less \{\}. Do I prefer more \{\}? & False\\
& I prefer more \{\}. Do I prefer less \{\}? & False\\
 & I prefer more \{\}. Do I prefer more \{\}? & True\\
\bottomrule
\end{tabular}

%%% Local Variables:
%%% mode: latex
%%% TeX-engine: xetex
%%% TeX-master: "../lrec-coling2024"
%%% End:


==> tables/results_by_context.tex <==
\begin{tblr}{lrrrrr}
\toprule
model & count & mass & intrans & trans & inchoative \\
\midrule
falcon & 0.81 & 0.58 & 0.84 & 0.70 & 0.78 \\
gpt-3.5 & 0.90 & 0.92 & 0.90 & 0.78 & 0.90 \\
gpt-4 & 1.00 & 0.99 & 0.87 & 0.99 & 0.99 \\
llama2 & 0.72 & 0.83 & 0.64 & 0.70 & 0.54 \\
mistral & 0.75 & 0.68 & 0.79 & 0.64 & 0.71 \\
\bottomrule
\end{tblr}

%%% Local Variables:
%%% mode: latex
%%% TeX-engine: xetex
%%% TeX-master: "../lrec-coling2024"
%%% End:


==> tables/results_by_typ_all.tex <==
\begin{tabular}{lcccccccccccc}
\toprule
&\multicolumn{3}{c}{count} & \multicolumn{3}{c}{mass} & \multicolumn{3}{c}{intrans} & \multicolumn{3}{c}{trans} \\
&  p & np & no & p & np & no & p & p & no & trans-p & np & no \\
\midrule
gpt-3.5 & 0.96 & 0.85 & 0.89 & 0.95 & 0.91 & 0.91 & 0.90 & 0.90 & 0.90 & 0.87 & 0.74 & 0.75 \\
gpt-4 & 1.00 & 0.99 & 1.00 & 0.99 & 0.98 & 1.00 & 0.89 & 0.88 & 0.84 & 1.00 & 0.99 & 0.99 \\
\midrule
falcon & 0.78 & 0.67 & 0.73 & 0.25 & 0.12 & 0.08 & 0.90 & 0.74 & 0.82 & 0.73 & 0.58 & 0.55 \\
llama2 & 0.69 & 0.68 & 0.71 & 0.80 & 0.75 & 0.82 & 0.60 & 0.60 & 0.60 & 0.68 & 0.63 & 0.65 \\
mistral & 0.68 & 0.61 & 0.67 & 0.46 & 0.42 & 0.40 & 0.68 & 0.59 & 0.65 & 0.52 & 0.47 & 0.49 \\\bottomrule
\end{tabular}

%%% Local Variables:
%%% mode: latex
%%% TeX-engine: xetex
%%% TeX-master: "../lrec-coling2024"
%%% End:


==> tables/results_by_typ_nonnull.tex <==
\begin{tabular}{lcccccccccccc}
\toprule
&\multicolumn{3}{c}{count} & \multicolumn{3}{c}{mass} & \multicolumn{3}{c}{intrans} & \multicolumn{3}{c}{trans} \\
&  p & np & no & p & np & no & p & p & no & trans-p & np & no \\
  \midrule
  gpt-3.5 & 0.96 & 0.85 & 0.89 & 0.95 & 0.91 & 0.91 & 0.90 & 0.90 & 0.90 & 0.87 & 0.74 & 0.75 \\
  gpt-4 & 1.00 & 0.99 & 1.00 & 0.99 & 1.00 & 1.00 & 0.89 & 0.88 & 0.84 & 1.00 & 0.99 & 0.99 \\
  \midrule
  falcon & 0.84 & 0.80 & 0.85 & 0.88 & 0.83 & 0.80 & 0.91 & 0.78 & 0.85 & 0.88 & 0.79 & 0.82 \\
  llama2 & 0.74 & 0.71 & 0.74 & 0.86 & 0.82 & 0.86 & 0.71 & 0.66 & 0.67 & 0.73 & 0.70 & 0.74 \\
  mistral & 0.85 & 0.82 & 0.87 & 0.82 & 0.81 & 0.76 & 0.94 & 0.92 & 0.95 & 0.69 & 0.70 & 0.69 \\
\bottomrule
\end{tabular}

%%% Local Variables:
%%% mode: latex
%%% TeX-engine: xetex
%%% TeX-master: "../lrec-coling2024"
%%% End:


==> tables/results_summary.tex <==
\begin{tblr}{lrrrrr}
\toprule
category & falcon & gpt-3.5 & gpt-4 & llama2 & mistral \\
\midrule
prototypical POS & 0.79 & 0.92 & 0.98 & 0.74 & 0.72 \\
\midrule
nonce word & 0.72 & 0.85 & 0.96 & 0.71 & 0.71 \\
non-prototypical POS & 0.70 & 0.84 & 0.97 & 0.71 & 0.69 \\
\bottomrule
\end{tblr}

%%% Local Variables:
%%% mode: latex
%%% TeX-engine: xetex
%%% TeX-master: "../lrec-coling2024"
%%% End:

